FedChain: Chained Algorithms for Near-Optimal Communication Cost in Federated Learning

Federated learning (FL) aims to minimize the communication complexity of training a model over heterogeneous data distributed across many clients. A common approach is local methods, where clients take multiple optimization steps over local data before communicating with the server (e.g., FedAvg). Local methods can exploit similarity between clients' data. However, in existing analyses, this comes at the cost of slow convergence in terms of the dependence on the number of communication rounds R. On the other hand, global methods, where clients simply return a gradient vector in each round (e.g., SGD), converge faster in terms of R but fail to exploit the similarity between clients even when clients are homogeneous. We propose FedChain, an algorithmic framework that combines the strengths of local methods and global methods to achieve fast convergence in terms of R while leveraging the similarity between clients. Using FedChain, we instantiate algorithms that improve upon previously known rates in the general convex and PL settings, and are near-optimal (via an algorithm-independent lower bound that we show) for problems that satisfy strong convexity. Empirical results support this theoretical gain over existing methods.

==> convex.tex <==
%!TEX root = ./main.tex
\section{Convex Rates}
% \begin{itemize}
%     \item General proof strategy: gradient norm bound of the second stage takes the function value progress of the first 
%     \item Rate for FedAvg
%     \item Rate for FedAvg$\to$SGD
%     \item Rate for FedAvg$\to$AGD
% \end{itemize}
% \begin{table*}
% 	\centering
% 	\renewcommand{\arraystretch}{1.4}
% 	\caption{Convergence rates of sub-optimality gap under general convexity, hiding constants and log terms.  For simplicity, $K$ is taken large enough to match the dominating terms in $R$ for all rates to emphasize the communication complexities of the algorithms given fast local computation.
% 	``X $ \to$ Y'' denotes first running ``X'' and using the output as input to ``Y''.  All rates achieved by \Lsgd$\to$X for some algorithm X can also achieved by SCAFFOLD$\to$X, given appropriate stepsize choice. 
% 	}
% 	\begin{tabular}{ l l }
% 	\hline 
% 	\textbf{Method/Analysis}  & \textbf{Sub-optimality rate:} $\mathbb{E} F(\hat{x}) - F(x^*)  \leq \tilde{\mathcal O}(\cdot)$ 
% 	\\ \hline
% 	\textit{ Centralized Algorithms} \\
% 	\hline
% 	\begin{tabular}{l} 
% 		\Mbsgd \\
% 		\asg \\
% 	\end{tabular}
% 	& \begin{tabular}{l}
% 		$\frac{\beta D^2}{R}$
% 		\\
% 		$\frac{\beta D^2}{R^2}$
% 		\\
% 	\end{tabular}
% 	\\\hline
% 	\textit{ Federated Algorithms} \\
% 	\hline
% 	\begin{tabular}{l}
% 		SCAFFOLD { \small \cite{karimireddy2020scaffold}} \\
% 		\Lsgd~{\small\cite{gorbunov2020local}}  \\
% 		%SCAFFOLD (Theorem \ref{thm:sslsgd}) \\
% 		\Lsgd $\to$ \Mbsgd (Theorem \ref{thm:twostageSGD})\\
% 		\Lsgd $\to$ \asg (Theorem \ref{thm:twostageasg})\\
% 		%M-\Lsgd $\to$ M-ASG \\  { (Theorem \ref{thm:multistageasg})}\\
% 		% Lower bound { \small\citep{woodworth2020minibatch}}
% 	\end{tabular}
% 	&
% 	\begin{tabular}{l}
		
% 		$\frac{\beta D^2}{R}$ 
% 		\\
% 		$\frac{\beta^{1/3} \zeta^{2/3} D^{4/3}}{R^{2/3}}$ \\
% 		%$\frac{\beta \zeta^2}{\mu^2 R^2}$ \\
% 		$\frac{\beta^{2/3} \zeta^{1/3} D^{5/3}}{R^{5/6}}$ \\
% 		$\frac{\beta^{2/3} \zeta^{1/3} D^{5/3}}{R^{4/3}}$ \\
% 		%$\min\{\Delta, \frac{\beta^2 \zeta^2}{\mu^3 R^2} + %\kappa \Delta \exp(-R)\}\exp(-\frac{R}{\sqrt{\kappa}}) + \frac{\sigma^2}{\mu N K R}$ \\ $[R \geq \Omega(\sqrt{\kappa})]$ \\
% 		% $\min\{\frac{\Delta}{\sqrt{\kappa}}, \frac{\mu \zeta^2_*}{\beta^2}\} \exp(-\frac{R}{\sqrt{\kappa}}) + \frac{\sigma^2}{\mu N K R}$ \\
% 	\end{tabular}
% 	\\\hline 
% \end{tabular}
% \label{tab:convexrates}
% \end{table*}

% \begin{table*}
% 	\centering
% 	\renewcommand{\arraystretch}{1.4}
% 	\caption{Convergence rates of gradient norm under general convexity, hiding constants and log terms.  For simplicity, $K$ is taken large enough to match the dominating terms in $R$ for all rates to emphasize the communication complexities of the algorithms given fast local computation.
% 	``X $ \to$ Y'' denotes first running ``X'' and using the output as input to ``Y''.  All rates achieved by \Lsgd$\to$X for some algorithm X can also achieved by SCAFFOLD$\to$X, given appropriate stepsize choice. $X$ + refers to running $X$ after adding a specific amount of regularization to the objective.
% 	}
% 	\begin{tabular}{ l l }
% 	\hline 
% 	\textbf{Method/Analysis}  & \textbf{Gradient Norm Rate:} $\mathbb{E} \|\nabla F(\hat{x})\|^2  \leq \tilde{\mathcal O}(\cdot)$ 
% 	\\ \hline
% 	\textit{ Centralized Algorithms} \\
% 	\hline
% 	\begin{tabular}{l} 
%         $\text{\mbsgd}^{\text{grad}}$   \\
%         $\text{\asg}^{\text{grad}}$ 
% 	\end{tabular}
% 	& \begin{tabular}{l}
% 		$\frac{\beta^2 D^2}{R^2}$
% 		\\
%         $\frac{\beta^2 D^2}{R^4}$
% 	\end{tabular}
% 	\\\hline
% 	\textit{ Federated Algorithms} \\
% 	\hline
% 	\begin{tabular}{l}
%         $\text{SCAFFOLD}^{\text{grad}}$ { \small\cite{karimireddy2020scaffold}} \\
%         $\text{\lsgd}^{\text{grad}}$ { \small\pcref{thm:informal-convex-lsgd-lsgd}}\\
% 		\Lsgd $\to$ \Mbsgd { \small\pcref{thm:informal-convex-lsgd-sgd}}\\
% 		\Lsgd $\to$ \asg { \small\pcref{thm:informal-convex-lsgd-asg}}\\
% 	\end{tabular}
% 	&
% 	\begin{tabular}{l}
%         $\frac{\beta^2 D^2}{R^2}$ \\
%         $\frac{\beta^{8/9} \zeta^{10/9} D^{8/9}}{R^{10/9}}$ \\
% 		$\min \{\frac{\beta^{4/3} \zeta^{2/3} D^{4/3}}{R^{5/3}}, \frac{\beta^2 D^2}{R^2} \}$ \\
% 		$\min \{\frac{\beta^{4/3} \zeta^{2/3} D^{4/3}}{R^{8/3}}, \frac{\beta^2 D^2}{R^4} \}$ \\
% 	\end{tabular}
% 	\\\hline 
% \end{tabular}
% \label{tab:convex-grad-rates}
% \end{table*}
Next we consider the case when $F_i$'s are general convex (i.e. strongly convex with $\mu=0$).  As in \cref{sec:strong}, the analysis in this section will focus on using \lsgd as $\ahead$, though one can also use SCAFFOLD with small modifications in the analysis.  We will first analyze the convergence rates of our chaining algorithms against baselines in terms of $\| \nabla F(\hat{x})\|^2$ and will later consider the optimality gap $F(\hat{x}) - F(x^*)$, where $\hat{x}$ is the returned iterate.  The gradient norm criterion is useful for a few reasons.  First, Nesterov \citep{nesterov2012make} argued that gradient norm guarantees can be more useful than function value guarantees for linearly constrained optimization problems which often arise in applications.  Second, the gradient norm is readily available to first-order algorithms as a stopping criterion, while suboptimality gap requires knowledge of $F(x^*)$.  Thus gradient norm guarantees can be more useful in practice.  Furthermore, gradient norm guarantees can be converted into suboptimality gap guarantees, provided that the algorithm does not increase distance to the optimal solution set by more than a constant factor, as we will discuss later.  We start by stating the known baselines for gradient norm minimization.  Analysis for gradient norm convergence already exists in the centralized setting:
\begin{fact}
	\label{fact:convex-sgd-grad}
	Suppose we run \mbsgd \pcref{algo:mbsgd} under the setting in \cite{woodworth2020minibatch} Theorem 1, and initialize another run of \mbsgd \pcref{algo:mbsgd} on the solution from the previous run of \mbsgd under the stepsize choice of \cref{prop:convex-sgd}, then we have 
	\begin{align*}
		\E \|\nabla F(\hat{x}) \|^2 \leq \tilde{\mathcal{O}}(\frac{\beta^2 D^2}{R^2} + \frac{\beta \sigma D}{\sqrt{NKR}})
	\end{align*}
	we will refer to this algorithm as $\text{\mbsgd}^{\text{grad}}$.  Suppose we run \asg \pcref{algo:ambsgd} under the setitng in \cite{woodworth2020minibatch} Theorem 1, and initialize another run of \asg \pcref{algo:ambsgd} on the solution from the previous run of \asg under the stepsize choice of \cref{prop:appasgconvex}, we have 
	\begin{align*}
		\E \|\nabla F(\hat{x})\|^2 \leq \tilde{\mathcal{O}}(\frac{\beta^2 D^2}{R^4} + \frac{\beta \sigma D}{\sqrt{NKR}} + \frac{\sigma^2}{NKR})
	\end{align*}
	We will refer to this baseline as $\text{\asg}^{\text{grad}}$.
\end{fact}
Note that these guarantees are stronger than what one would get from simply applying smoothness to suboptimality gap guarantees for \mbsgd or \asg.  For example, when $\sigma^2 = 0$, the suboptimality gap guarantee for \mbsgd is $\frac{\beta D^2}{R}$ \cite{woodworth2020minibatch}, and applying smoothness via $\|\nabla F(x)\|^2 \leq 2 \beta(F(x) - F(x^*))$ would give a worse rate than is given in \cref{fact:convex-sgd-grad}.  Next, we develop the other baseline, \lsgd:
\begin{theorem}[Informal version of \cref{thm:convex-lsgd-lsgd}]
	\label{thm:informal-convex-lsgd-lsgd}
	Suppose we first run \lsgd \pcref{algo:fedavg}, and use its solution as the initialization of a regularized version of \lsgd \pcref{algo:fedavg}, under some parameter settings including the amount of regularization.  Then the solution $\hat{x}$ of this algorithm has 
	\begin{align*}
		&\E \|\nabla F(\hat{x}) \|^2 \leq \tilde{\mathcal{O}}(\frac{\beta^{8/9} \zeta^{10/9} D^{4/9}}{R^{10/9}} + \frac{\beta \sigma D}{\sqrt{NKR}} + \textup{Err})
	\end{align*}
	where $\textup{Err}$ represents other lower order/decreasing with $K$ additive error terms that we leave out to simplify comparison with our chaining \pcref{algo:chaining} algorithms.  We will call this algorithm $\text{\lsgd}^{\text{grad}}$.
\end{theorem}
To see why this guarantee is better than simply applying smoothness to the suboptimality gap guarantee, first set $\beta = D = 1$ for simplicity, and disregard any terms that decrease with $K$.  Then the suboptimality gap for \lsgd is $\frac{\zeta^{2/3}}{R^{2/3}}$.  Applying smoothness, the gradient norm guarantee is again $\frac{\zeta^{2/3}}{R^{2/3}}$.  Now turn to our rate for $\text{\lsgd}^{\text{grad}}$ \pcref{thm:informal-convex-lsgd-lsgd}: $\frac{\zeta^{10/9}}{R^{10/9}}$.  For either rate to be better than the \asg rate of $\frac{1}{R^4}$ \pcref{fact:convex-sgd-grad}, we need that $\zeta << 1$, and so increasing the exponents for $\zeta$ and $R$ are both improvements.  To our knowledge, the rate in \cref{thm:informal-convex-lsgd-lsgd} is the best gradient norm guarantee for \lsgd in terms of communication round complexity, given large enough $K$.  Next, we give the guarantee for \chain{\lsgd}{\mbsgd} under the general convex assumption.
\begin{theorem}[Informal version of \cref{thm:convex-lsgd-sgd}]
	\label{thm:informal-convex-lsgd-sgd}
	Suppose we run \cref{algo:chaining} where $\ahead$ is \lsgd \cref{algo:fedavg} under some parameter settings for $R/2$ rounds and $\atail$ is \mbsgd \cref{algo:mbsgd} $R/2$ rounds under some other parameter settings.  Then we have:
	\begin{align*}
		&\E \|F (\hat{x}_2)\|^2 \\
		&\leq \tilde{\mathcal{O}}(\min\{\frac{\beta^{4/3} \zeta^{2/3} D^{4/3}}{R^{5/3}} + \frac{\beta}{R}\errk{convex}, \frac{\beta^2 D^2}{R^2}\}) \\
		&+ \tilde{\mathcal{O}}( \frac{\beta \sigma D}{\sqrt{NKR}})
	\end{align*}
	where $\errk{convex} =  \frac{\beta D^2}{K R} + \frac{\beta^{1/3} \sigma^{2/3} D^{4/3}}{K^{1/3} R^{2/3}} + \frac{\sigma}{\sqrt{NK} }$.
	We will refer to this algorithm as \chain{\lsgd}{\mbsgd}.
\end{theorem}
\begin{corollary}
	\label{cor:convex-lsgd-sgd}
	Suppose

	$K \geq \max \{\frac{\beta^{2/3} D^{2/3}}{\zeta^{2/3}R^{1/3}}, \frac{\sigma^2}{\zeta^2}, \frac{\sigma^2 R^{4/3}}{\zeta^{4/3} \beta^{2/3} D^{8/3} N^{1/2}}\}$ in the setting of \cref{thm:informal-convex-lsgd-sgd}, then we have 
	\begin{align*}
		&\E \|F (\hat{x}_2)\|^2 \\
		&\leq \tilde{\mathcal{O}}(\min\{\frac{\beta^{4/3} \zeta^{2/3} D^{4/3}}{R^{5/3}}, \frac{\beta^2 D^2}{R^2}\}+ \frac{\beta \sigma D}{\sqrt{NKR}}) 
	\end{align*}
\end{corollary}
We now compare the converence rate of \chain{\lsgd}{\mbsgd} \pcref{cor:convex-lsgd-sgd} to that of $\text{\mbsgd}^{\text{grad}}$ \pcref{fact:convex-sgd-grad} and $\text{\lsgd}^{\text{grad}}$ \pcref{thm:informal-convex-lsgd-lsgd}.  First, observe that the variance term in \chain{\lsgd}{\mbsgd} matches the same variance term those of $\text{\mbsgd}^{\text{grad}}$ \pcref{fact:convex-sgd-grad} and $\text{\lsgd}^{\text{grad}}$ \pcref{thm:informal-convex-lsgd-lsgd}.  Now we compare the terms that only decrease with $R$.  For simplicity, set $D = \beta = 1$.  The $\min\{\frac{\zeta^{2/3} }{R^{5/3}}, \frac{1}{R^2}\}$ term of \chain{\Lsgd}{\mbsgd} is at least as good as the $\frac{1}{R^2}$ term of $\text{\mbsgd}^{\text{grad}}$ \pcref{fact:convex-sgd-grad} in all cases, and is in particular strictly better if $\zeta < \frac{1}{R^{1/2}}$.  On the other hand, the $\min\{\frac{\zeta^{2/3} }{R^{5/3}}, \frac{1}{R^2}\}$ term of \chain{\Lsgd}{\mbsgd} term of \chain{\lsgd}{\mbsgd} is better than the $\frac{\zeta^{10/9}}{R^{10/9}}$ term of $\text{\lsgd}^{\text{grad}}$ if $\zeta > \frac{1}{R^{5/4}}$.  Taken together, unfortunately there is no regime of $\zeta$ in which \chain{\lsgd}{\mbsgd} is the best algorithm.  This underperformance can be addressed via acceleration in the next theorem.
\begin{theorem}[Informal version of \cref{thm:convex-lsgd-asg}]
	\label{thm:informal-convex-lsgd-asg}
	Suppose we run \cref{algo:chaining} where $\ahead$ is \lsgd \cref{algo:fedavg} under some parameter settings for $R/2$ rounds and $\atail$ is \asg \cref{algo:ambsgd} $R/2$ rounds under some other parameter settings.  Then we have:
	\begin{align*}
		&\E \|F (\hat{x}_2)\|^2 \leq \\
		&\tilde{\mathcal{O}}(\min\{\frac{\beta^{4/3} \zeta^{2/3} D^{4/3}}{R^{8/3}} + \frac{\beta}{R^2} \errk{convex}, \frac{\beta^2 D^2}{R^4}\}) \\
		&+ \tilde{\mathcal{O}}(\frac{\beta \sigma D}{\sqrt{NKR}} + \frac{\sigma^2}{NKR})
	\end{align*}
	Where $\errk{convex}$ was defined in \cref{thm:informal-convex-lsgd-sgd}.  We refer to this algorithm as \chain{\lsgd}{\asg}.
\end{theorem}
\begin{corollary}
	\label{cor:convex-lsgd-asg}
	Suppose

	$K \geq \max \{\frac{\beta^{2/3} D^{2/3}}{\zeta^{2/3}R^{1/3}}, \frac{\sigma^2}{\zeta^2}, \frac{\sigma^2 R^{4/3}}{\zeta^{4/3} \beta^{2/3} D^{8/3} N^{1/2}}\}$ in the setting of \cref{thm:informal-convex-lsgd-sgd}, then we have 
	\begin{align*}
		&\E \|F (\hat{x}_2)\|^2 \\
		&\leq \tilde{\mathcal{O}}(\min\{\frac{\beta^{4/3} \zeta^{2/3} D^{4/3}}{R^{8/3}}, \frac{\beta^2 D^2}{R^4}\}) \\
		&+\tilde{\mathcal{O}}(\frac{\beta \sigma D}{\sqrt{NKR}} + \frac{\sigma^2}{NKR})
	\end{align*}
\end{corollary}
Again let us assume $\beta = D = 1$ for simplicity.  Then the variance terms ``match'' across all algorithms: they all have the term $\frac{\sigma}{\sqrt{NKR}}$, and the term $\frac{\sigma^2}{NKR}$ of \chain{\lsgd}{\asg} has the same round complexity to reach $\epsilon$ error as $\frac{\sigma}{\sqrt{NKR}}$.  Next we discuss the terms that only decrease with $R$.  Then the $\min\{ \frac{\zeta^{2/3} }{R^{8/3}}, \frac{1}{R^4}\}$ term of \chain{\lsgd}{\asg} is strictly better than $\text{\asg}^{\text{grad}} $ if $\zeta < \frac{1}{R^2}$.  On the other hand, the $\min\{ \frac{\zeta^{2/3} }{R^{8/3}}, \frac{1}{R^4}\}$ term of \chain{\lsgd}{\asg} is better than $\text{\lsgd}^{\text{grad}}$ if $\zeta > \frac{1}{R^{7/2}}$.  Altogether, this gives a regime $\frac{1}{R^{7/2}} < \zeta < \frac{1}{R^{2}}$ where \chain{\lsgd}{\asg} is the most communication-efficient algorithm under the gradient norm convergence criterion.

Next we discuss converting the gradient norm guarantees into suboptimality gap.  It can be shown (as proven in the formal versions of \cref{thm:informal-convex-lsgd-sgd} and \cref{thm:informal-convex-lsgd-asg}) that both \chain{\lsgd}{\mbsgd} and \chain{\lsgd}{\asg} do not increase the distance from the optimum by more than a log factor.  We focus on \chain{\lsgd}{\asg} from here on out.  Ignoring the terms that decrease with $K$, we have that 
\begin{align*}
	\E \|F(\hat{x}_2)\|^2 \leq \tilde{\mathcal{O}}(\min\{\frac{\beta^{4/3} \zeta^{2/3} D^{4/3}}{R^{8/3}}, \frac{\beta^2 D^2}{R^4}\})
\end{align*}
From convexity, we know that 
\begin{align*}
	&F(\hat{x}_2) - F(x^*) \\
	&\leq \langle \nabla F(\hat{x}_2), \hat{x}_2 - x^* \rangle \leq \|\nabla F(\hat{x}_2)\| \|\hat{x}_2 - x^*\|
\end{align*}
And plugging our result for gradient norm in and noting that $\|\hat{x}_2 - x^*\| \leq \tilde{\mathcal{O}}(\|\hat{x}_0 - x^*\|)$,
\begin{align*}
	F(\hat{x}_2) - F(x^*) \leq \tilde{\mathcal{O}}(\min\{\frac{\beta^{2/3} \zeta^{1/3} D^{5/3}}{R^{4/3}}, \frac{\beta D^2}{R^2}\})
\end{align*}
The rate on the right side of the $\min$ is the \asg suboptimality gap, and the rate on the left side is in fact $ab$, where $a^2 = \frac{\beta^{1/3} \zeta^{2/3} D^{4/3}}{R^{2/3}}$, the only term from \lsgd's \pcref{algo:fedavg} convergence rate that does not decrease with $K$ \cite{woodworth2020minibatch} in the general convex setting and $b^2 = \frac{\beta D^2}{R^2}$, which is the only term from \asg's \pcref{algo:ambsgd} convergence rate that does not decrease with $K$ \cite{woodworth2020minibatch}.  $ab$ is the geometric mean of $a^2$ and $b^2$, and so our rate for \chain{\lsgd}{\asg} for the suboptimality gap does not have any regime in which it improves over both \lsgd and \asg.  

Altogether, the gains in the general convex section by our chaining framework \pcref{algo:chaining} are more muted than in the strongly convex case: we make convergence rate gains under the gradient norm convergence criterion, but are unable to prove gains under the suboptimality gap.  


==> pl.tex <==
%!TEX root = ./main.tex
\section{Nonconvex Rates}
% \begin{itemize}
% 	\item General proof strategy: function value bound from the first stage can be plugged into the function value bound of the second stage 
% 	\item Our rate for FedAvg 
% 	\item Rate for FedAvg$\to$SGD
% \end{itemize}
% \begin{table*}
% 	\centering
% 	\renewcommand{\arraystretch}{1.4}
% 	\caption{Convergence rates of gradient norm under $\mu$-PL condition, hiding constants and log terms.  For simplicity, $K$ is taken large enough to match the dominating terms in $R$ for all rates to emphasize the communication complexities of the algorithms given fast local computation.
% 	``X $ \to$ Y'' denotes first running ``X'' and using the output as input to ``Y''.  All rates achieved by \Lsgd$\to$X for some algorithm X can also achieved by SCAFFOLD$\to$X, given appropriate stepsize choice. 
% 	}
% 	\begin{tabular}{ l l }
% 	\hline 
% 	\textbf{Method/Analysis}  & \textbf{Sub-optimality rate:} $\mathbb{E} F(\hat{x}) - F(x^*)  \leq \tilde{\mathcal O}(\cdot)$ 
% 	\\ \hline
% 	\textit{ Centralized Algorithms} \\
% 	\hline
% 	\begin{tabular}{l} 
% 		\Mbsgd \pcref{thm:plsgd} \\
% 	\end{tabular}
% 	& \begin{tabular}{l}
% 		$\Delta \exp(- \frac{R}{\kappa})$
% 		\\
% 	\end{tabular}
% 	\\\hline
% 	\textit{ Federated Algorithms} \\
% 	\hline
% 	\begin{tabular}{l}
% 		\Lsgd \cite{karimireddy2020mime} \\
% 		\Lsgd $\to$ \Mbsgd \pcref{thm:informal-pl-lsgd-sgd}\\
% 		M-\Lsgd $\to$ M-\Mbsgd \pcref{thm:pl-mlsgd-msgd} \\
% 		%MimeMVR \cite{karimireddy2020mime}
% 	\end{tabular}
% 	&
% 	\begin{tabular}{l}
% 		$\kappa \Delta \exp(- \frac{R}{\kappa})  + \kappa^2 (\frac{\zeta^2}{\mu}) R^{-2} $ \\
%         $\min \{\frac{\zeta^2}{\mu}, \Delta \} \exp(- \frac{R}{\kappa})$ \\
% 		$\min \{\kappa^2 \frac{\zeta^2}{\mu}, \Delta \} \exp(- \frac{R}{\kappa})$ \ \ \ for $R \geq \Omega(\kappa)$\\
% 		%$(\frac{\delta}{\mu}) \Delta R^{-1} + (\frac{\delta^2 \zeta^2 \Delta^2}{\mu^3})^{1/3}N^{-1/3} R^{2/3} + (\frac{\zeta^2}{\mu})N^{-1} R^{-1} $
% 	\end{tabular}
% 	\\\hline 
% \end{tabular}
% \label{tab:pl-rates}
% \end{table*}
In this section, we go beyond convexity to show that our chaining framework \pcref{algo:chaining} can achieve significant gains over existing federated optimization baselines under the $\mu$-PL condition. \footnote{We abuse notation and use the same $\mu$ for both strong convexity and PL--this is standard as strong convexity actually implies PL.  However the opposite is not true: the PL condition is much weaker than strong convexity \cite{karimi2016linear}.}  Afterwards, we will discuss the performance of the chaining framework in the general nonconvex setting.
\begin{definition}
	$F$ is considered $\mu$-PL if we have that for any $x$,
	\begin{align*}
		2\mu(F(x) - F(x^*)) \leq \|\nabla F(x)\|^2
	\end{align*}
\end{definition}
Throughout this section, we will assume that $F$ (not necessarily $F_i$'s) is $\mu$-PL.  The PL condition characterizes many machine learning problems, such as least squares and logistic regression \cite{karimi2016linear} and natural parameterizations of problems in reinforcement learning \cite{pmlr-v80-fazel18a} \cite{agarwal2021theory} \cite{bhandari2019global} (it is referred to as gradient domination in this setting).  We start by writing the convergence rates for the baselines in this setting.
\begin{fact}
	\label{fact:pl-sgd-lsgd}
	If we run \lsgd in the setting of \cite{karimireddy2020mime}, then we have convergence rate 
	\begin{align}
		F(\hat{x}) - F(x^*) \leq \Delta \exp(-\frac{R}{\kappa}) + \frac{\kappa \zeta^2}{\mu R^2} + \frac{\sigma^2}{\mu R}
	\end{align}
	and if we run \mbsgd under the setting of \cref{thm:plsgd}, we have convergence rate
	\begin{align}
		F(\hat{x}) - F(x^*) \leq \Delta \exp(-\frac{R}{\kappa}) + \frac{\kappa \sigma^2}{\mu N K R}
	\end{align}
\end{fact}
Under current analysis done for \lsgd under the $\mu$-PL condition, \lsgd is so far unable to achieve constant communication round complexity supposing that $\zeta = 0$.  So disregarding the terms that decrease with $K$, we can see that the guarantee for \mbsgd actually dominates the guarantee for \lsgd under the PL condition.  We will show that using our chaining framework \pcref{algo:chaining}, we can improve upon these rates substantially.
\begin{theorem}[Informal version of \cref{thm:pl-lsgd-sgd} in Appendix]
	\label{thm:informal-pl-lsgd-sgd}
	Suppose we run \cref{algo:chaining} where $\ahead$ is \lsgd \pcref{algo:fedavg} under some parameter settings for $R/2$ rounds and $\atail$ is \mbsgd \pcref{algo:mbsgd} under some other parameter settings for $R/2$ rounds, we have 
	\begin{align*}
		&\E F(\hat{x}_2) - F(x^*) \leq\\
		&\tilde{\mathcal{O}}((\min \{ \frac{\zeta^2}{\mu} + \errk{chain}, \Delta\} + \frac{\sigma}{\sqrt{NK}})\exp(-\frac{R}{\kappa})) \\
		&+ \tilde{\mathcal{O}}(\frac{\kappa \sigma^2}{\mu N K R})
	\end{align*}
	where $\errk{chain} = \Delta \exp(-\frac{R \sqrt{K}}{\kappa}) + \frac{\sigma^2}{\mu \sqrt{K}}$.  We will refer to this algorithm as \chain{\lsgd}{\mbsgd}.
\end{theorem}
\begin{corollary}
	\label{cor:informal-pl-lsgd-sgd}
	$K \geq \max \{\frac{\kappa^2}{R^2} \log^2(\frac{\mu \Delta}{\zeta^2}), \frac{\sigma^4}{\zeta^4}, \frac{\sigma^2}{\Delta^2 N^2}, \frac{\mu^2 \sigma^2}{\zeta^4 N}\}$, then the algorithm specified in \cref{thm:informal-convex-lsgd-sgd} has convergence rate
	\begin{align*}
		&\E F(\hat{x}_2) - F(x^*) \leq\\
		&\tilde{\mathcal{O}}(\min \{ \frac{\zeta^2}{\mu}, \Delta\}\exp(-\frac{R}{\kappa}) + \frac{\kappa \sigma^2}{\mu N K R})
	\end{align*}
\end{corollary}
% \begin{theorem}[Informal version of \cref{thm:pl-mlsgd-msgd}]
% 	\label{thm:informal-pl-mlsgd-msgd}
% 	Suppose we run \cref{algo:chaining}:
% 	\begin{enumerate}
% 		\item Where $\ahead$ is M-\lsgd \pcref{algo:m-lsgd}, a stepsize decaying version of \Lsgd
% 		\item Where $\atail$ is either M-\mbsgd \pcref{algo:m-mbsgd} which is a stepsize decaying version of \mbsgd \pcref{algo:mbsgd}
% 	\end{enumerate}
% 	Then M-\lsgd $\to$ M-\mbsgd recovers the same convergence rate as \lsgd $\to$ \mbsgd \pcref{thm:informal-pl-lsgd-sgd}
% \end{theorem}
Let us consider the terms that do not decrease with $K$.  Then the term $\min \{ \frac{\zeta^2}{\mu}, \Delta\}\exp(-\frac{R}{\kappa})$ is smaller than the $\Delta \exp(-\frac{R}{\kappa})$ terms of both \lsgd and \mbsgd \pcref{fact:pl-sgd-lsgd}.  For terms that do decrease with $K$, the $\frac{\kappa\sigma^2}{\mu N K R}$ term of \chain{\lsgd}{\mbsgd} matches that of \mbsgd.  There are no terms that decrease with $K$ for the rate of \lsgd.  We end discussion of the $\mu$-PL setting that we can also have stepsize scheduling here as well, similar to the strongly convex setting: see \cref{thm:pl-mlsgd-msgd}.

Next we discuss the general nonconvex setting.  For simplicity, let $\sigma^2 = 0$.  Using smoothness and the bound on heterogeneity, we can show that after one communication round and $K$ local steps sampled on one client\footnote{In analysis for federated optimization in the nonconvex setting, it is common to only sample one client or assume weak convexity to prevent averaging from blowing up the loss \cite{karimireddy2020mime}.  We do have an analysis that allows averaging in the nonconvex case \cref{thm:fedavgpl-convergent}, though it loses factors of $\beta$.} following the analysis of \cref{thm:fedavgpl} without using the PL condition, where $x_k$ are the iterates of the client and $\eta \leq \frac{1}{\beta}$:
\begin{align*}
	F(\hat{x}_{1/2}) \leq F(\hat{x}_0) - \frac{\eta}{2} \sum_{k=1}^K \|\nabla F(x_k)\|^2 + \frac{\eta \zeta^2 K}{2}
\end{align*}
Assume that $F(\hat{x}_{1/2})< F(\hat{x}_0)$ for simplicity, and set $\hat{x}_1 = \hat{x}_{1/2}$.  Then if we run \mbsgd as $\atail$, by standard nonconvex analysis of \mbsgd run for $R$ rounds (let $\x{r}$ be \mbsgd's iterate at the $r+1$'th communication round and $\eta \leq \frac{1}{\beta}$)
\begin{align*}
	&F(\hat{x}_2) \leq F(\hat{x}_{1}) - \frac{\eta}{2}\sum_{r = 0}^{R-1} \|\nabla F(\x{r})\|^2 \\
	&\leq F(\hat{x}_0) - \frac{\eta}{2} \sum_{k=1}^K \|\nabla F(x_k)\|^2  - \frac{\eta}{2}\sum_{r = 0}^{R-1} \|\nabla F(\x{r})\|^2 \\
	& \ \ \ \ + \frac{\eta \zeta^2 K}{2}
\end{align*}
And choosing a uniformly sampled iterate from the $x_k$'s and $\x{r}$'s as $\bar{x}$ while also setting $\eta = \frac{1}{\beta}$ and noting $F(\hat{x}_2) \leq F(x^*)$,
\begin{align*}
	&\E \|\nabla F(\bar{x})\|^2 \\
	&\leq (\frac{1}{R + K})( \sum_{k=1}^K \|\nabla F(x_k)\|^2  + \sum_{r = 0}^{R-1} \|\nabla F(\x{r})\|^2) \\
	&\leq \frac{2(F(\hat{x}_0) - F(\hat{x}_2))}{\eta (R + K)} + \frac{\zeta^2 K}{R + K} \\
	&\leq \frac{2\beta(F(\hat{x}_0) - F(x^*))}{ (R + K)} + \frac{\zeta^2 K}{R + K}
\end{align*}
This rate has a nice property: given $\zeta^2$ on the order of $\epsilon$, one can get arbitraily low gradient norm with high $K$.  On the other hand, with a non-insignificant $\zeta$, it can still converge if we choose a $K$ that is of smaller order than $R$.  This, to our knowledge, is the first guarantee of its kind in the nonconvex federated learning optimization literature under our heterogeneity assumptions, which are standard in the federated learning literature \cite{woodworth2020minibatch} \cite{gorbunov2020local} \cite{kairouz2019advances}.  It is possible to obtain stronger guarantees given more assumptions, such as the Hessian heterogeneity assumption of \cite{karimireddy2020mime}.

Altogether, in the nonconvex setting the chaining framework was able to demonstrate strong improvements given the PL condition, and under general nonconvexity achieved a smaller improvement over previous baselines.

==> strong.tex <==
%!TEX root = ./main.tex
\section{Strongly Convex Rates}
\label{sec:strong}
We start by considering the performance of the chaining framework \pcref{algo:chaining} in the case where each $F_i$ is $\mu$-strongly convex.  The analysis in this section focuses on the use of \lsgd as $\ahead$, though one can also use SCAFFOLD \cite{karimireddy2020scaffold} with small modifications in the proofs.  For comparison purposes, we start by recalling the convergence rates of \lsgd and \mbsgd/\asg (Stochastic Gradient Descent and Accelerated Stochastic Gradient).
\begin{fact}[Informal version of Theorem 1 in \cite{woodworth2020minibatch}]
	\label{fact:sgd-strong}
	Suppose we run \mbsgd \pcref{algo:fedavg} under the parameter settings specified in Theorem 1 in \cite{woodworth2020minibatch}.  Then if the returned solution is $\hat{x}$, we have 
	\begin{align*}
		\E F(\hat{x}) - F(x^*) \leq \tilde{\mathcal{O}}(\kappa \Delta \exp(-\frac{R}{\kappa}) + \frac{\sigma^2}{\mu N K R}) 
	\end{align*}
	with acceleration, we have that 
	\begin{align*}
		\E F(\hat{x}) - F(x^*) \leq \tilde{\mathcal{O}}(\Delta \exp(-\frac{R}{\sqrt{\kappa}}) + \frac{\sigma^2}{\mu N K R}) 
	\end{align*}
	as long as $R \geq \Omega(\sqrt{\kappa})$.
\end{fact}
\begin{fact}[Informal version of Theorem G.3 in \cite{gorbunov2020local}]
	\label{fact:fedavg-strong}
	Suppose we run \lsgd \pcref{algo:fedavg} under the parameter settings specified in Theorem G.3 in \cite{gorbunov2020local}.  Then if the returned solution is $\hat{x}$, we have 
	\begin{align*}
		\E F(\hat{x}) - F(x^*) \leq \tilde{\mathcal{O}}(\kappa(\frac{\zeta^2}{\mu}) R^{-2} + \errk{\lsgd}) 
	\end{align*}
	where $\errk{\lsgd} := \kappa \Delta \exp(-\frac{KR}{\kappa}) + \frac{\sigma^2}{\mu N K R} + \frac{\kappa \sigma^2}{\mu K R^2}$.
\end{fact}
From \cref{fact:fedavg-strong}, we see that \lsgd's error depends on $\kappa (\frac{\zeta^2}{\mu}) R^{-2}$ which only shrinks with $R$ (communication rounds), and $\errk{\lsgd}$ which shrinks with $K$ (local computation) as well as $R$.  In particular, the $\kappa (\frac{\zeta^2}{\mu}) R^{-2}$ term is troubling for communication efficiency, because a rate of $R^{-2}$ is much slower compared to exponential rates that one would expect in the strongly convex setting.  In what follows, we see that by applying the chaining framework \pcref{algo:chaining}, one can improve the dependence on $\zeta^2$ (data heterogeneity) exponentially. 
\begin{theorem}[Informal version of \cref{thm:lsgd-sgd} in Appendix]
	\label{thm:informal-strong-lsgd-sgd}
	Suppose we run \cref{algo:chaining} where $\ahead$ is \lsgd \pcref{algo:fedavg} under some parameter settings for $R/2$ rounds and $\atail$ is \mbsgd \pcref{algo:mbsgd} under some other parameter settings for $R/2$ rounds, we have 
	\begin{align*}
		&\E F(\hat{x}_2) - F(x^*) \leq\\
		&\tilde{\mathcal{O}}((\min \{ \frac{\zeta^2}{\mu} + \errk{chain}, \Delta\} + \frac{\sigma}{\sqrt{NK}})\exp(-\frac{R}{\kappa})) \\
		&+ \tilde{\mathcal{O}}(\frac{\kappa \sigma^2}{\mu N K R})
	\end{align*}
	where $\errk{chain} = \Delta \exp(-\frac{R \sqrt{K}}{\kappa}) + \frac{\sigma^2}{\mu \sqrt{K}}$.
\end{theorem}
\begin{corollary}
	\label{cor:informal-strong-lsgd-sgd}
	$K \geq \max \{\frac{\kappa^2}{R^2} \log^2(\frac{\mu \Delta}{\zeta^2}), \frac{\sigma^4}{\zeta^4}, \frac{\sigma^2}{\Delta^2 N^2}, \frac{\mu^2 \sigma^2}{\zeta^4 N}\}$, then the algorithm specified in \cref{thm:informal-convex-lsgd-sgd} has convergence rate
	\begin{align*}
		&\E F(\hat{x}_2) - F(x^*) \leq\\
		&\tilde{\mathcal{O}}(\min \{ \frac{\zeta^2}{\mu}, \Delta\}\exp(-\frac{R}{\kappa}) + \frac{\kappa \sigma^2}{\mu N K R})
	\end{align*}
\end{corollary}
We will refer to the algorithm where we use \lsgd as $\ahead$ and \mbsgd as $\atail$ as \chain{\lsgd}{\mbsgd}.  Let us compare the rate in \cref{cor:informal-strong-lsgd-sgd} for \chain{\lsgd}{\mbsgd} to the rate of only \lsgd.  We start by comparing the terms that only shrink with $R$.  First observe that the $\min \{\frac{\zeta^2}{\mu}, \Delta\} \exp(-\frac{R}{\kappa})$ term in \cref{cor:informal-strong-lsgd-sgd} both (1) improves exponentially and (2) improves condition number factor-wise over the $\kappa (\frac{\zeta^2}{\mu}) R^{-2}$ term of \cref{fact:fedavg-strong}.  Next, observe that $\min \{\frac{\zeta^2}{\mu}, \Delta\} \exp(-\frac{R}{\kappa})$ is always better than the $\kappa \Delta \exp(-\frac{R}{\kappa})$ term of \mbsgd \pcref{fact:sgd-strong}, and is especially better if $\frac{\zeta^2}{\mu} << \Delta$.  So given arbitrary local computation, \chain{\lsgd}{\mbsgd} shows substantial improvement in communication complexity over existing baselines.

Next, we consider the terms that decrease with $K$ (local computation).  Comparing the $\frac{\kappa \sigma^2}{\mu N K R}$ term of \cref{cor:informal-strong-lsgd-sgd} to the $\frac{\kappa \sigma^2}{\mu K R^2}$ term of \lsgd \pcref{fact:fedavg-strong}, we see that unless $N \geq R$, the $\frac{\kappa \sigma^2}{\mu N K R}$ term of \cref{cor:informal-strong-lsgd-sgd} is worse.  $\frac{\kappa \sigma^2}{\mu N K R}$ also loses a condition number factor against the variance term of \mbsgd $\frac{\sigma^2}{\mu NKR}$ \pcref{fact:sgd-strong}.  The underperformance in the variance terms can be addressed via acceleration in the next theorem.
\begin{theorem}[Informal version of \cref{thm:lsgd-asg} in Appendix]
	\label{thm:informal-strong-lsgd-asg}
	Suppose we run \cref{algo:chaining} where $\ahead$ is \lsgd \pcref{algo:fedavg} under some parameter settings for $R/2$ rounds and $\atail$ is \asg \pcref{algo:ambsgd} under some other parameter settings for $R/2$ rounds, we have 
	\begin{align*}
		&\E F(\hat{x}_2) - F(x^*) \leq\\
		&\tilde{\mathcal{O}}((\min \{ \frac{\zeta^2}{\mu} + \errk{chain} , \Delta\}+ \frac{\sigma}{\sqrt{N K}}) \exp(-\frac{R}{\sqrt{\kappa}})) \\
		&+ \tilde{\mathcal{O}}(\frac{\sigma^2}{\mu N K R}+ \frac{\kappa\sigma^2}{\mu N K R^3})
	\end{align*}
	where $\errk{chain}$ was defined in \cref{thm:informal-strong-lsgd-sgd}.
\end{theorem}
\begin{corollary}
	\label{cor:informal-strong-lsgd-asg}
	$K \geq \max \{\frac{\kappa^2}{R^2} \log^2(\frac{\mu \Delta}{\zeta^2}), \frac{\sigma^4}{\zeta^4}, \frac{\sigma^2}{\Delta^2 N^2}, \frac{\mu^2 \sigma^2}{\zeta^4 N}\}$, then the algorithm specified in \cref{thm:informal-strong-lsgd-asg} has convergence rate
	\begin{align*}
		&\E F(\hat{x}_2) - F(x^*) \leq\\
		&\tilde{\mathcal{O}}(\min \{ \frac{\zeta^2}{\mu}, \Delta\}\exp(-\frac{R}{\sqrt{\kappa}}) +\frac{\sigma^2}{\mu N K R}+ \frac{\kappa\sigma^2}{\mu N K R^3})
	\end{align*}
\end{corollary}
The algorithm instantiated in \cref{thm:informal-strong-lsgd-asg} will be called \chain{\lsgd}{\asg}.  We start by comparing the terms that only decrease with $R$ and not $K$.  The $\min \{ \frac{\zeta^2}{\mu}, \Delta\}\exp(-\frac{R}{\sqrt{\kappa}})$ term of \chain{\lsgd}{\asg} \pcref{cor:informal-strong-lsgd-asg} is strictly better than the $\min \{ \frac{\zeta^2}{\mu}, \Delta\}\exp(-\frac{R}{\kappa})$ term of \chain{\lsgd}{\mbsgd}, and so by the earlier discussion on \cref{cor:informal-strong-lsgd-sgd}, \chain{\lsgd}{\asg} has the best dependence on terms that only shrink with $R$.

Next, we consider the terms that decrease with $K$.  First, observe that the $\frac{\sigma^2}{\mu N K R}$ of \cref{cor:informal-strong-lsgd-asg} matches the same terms terms in the rates of \lsgd \pcref{fact:fedavg-strong} and \asg \pcref{fact:sgd-strong}.  The $\frac{\kappa \sigma^2}{\mu N K R^3}$ term of \cref{cor:informal-strong-lsgd-asg} is strictly better than the $\frac{\kappa \sigma^2}{\mu K R^2}$ of \lsgd \pcref{fact:fedavg-strong} and given the round restriction on $R$ for \asg in \cref{fact:sgd-strong}, also matches the $\frac{\sigma^2}{\mu N K R}$ term of \asg.  On the other hand, the $\frac{\kappa \sigma^2}{\mu N K R^3}$ term is larger than the $\frac{\sigma^2}{\mu N K R}$ term of \mbsgd \cref{fact:sgd-strong}, but \mbsgd's rate requires $R > \kappa$ anyways to reach any given accuracy $\epsilon$--thus in this regime $\frac{\kappa \sigma^2}{\mu N K R^3} < \frac{\sigma^2}{\mu NKR}$.  In conclusion, given a lower bound requirement on $K$, \chain{\lsgd}{\asg} has the best convergence rate over all known baselines in terms of communication round complexity under the strongly convex conditions.

\underline{\textbf{Proof Sketch:}}  We will prove the convergence rate of \chain{\lsgd}{\mbsgd}.  The case for \chain{\lsgd}{\asg} is similar.

\textbf{1. Convergence rate of \lsgd used as $\ahead$:} One could use the convergence rate of \cite{gorbunov2020local} for \lsgd, which would give
\begin{align*}
	\E F(\hat{x}_{1/2}) - F(x^*) \leq \tilde{\mathcal{O}}(\kappa(\frac{\zeta^2}{\mu}) R^{-2} + \errk{\lsgd})
\end{align*}
where $\errk{\lsgd}$ was defined in \cref{fact:fedavg-strong}.  However, we prove a guarantee for \lsgd under a different stepsize choice 
\begin{align*}
	\E F(\hat{x}_{1/2}) - F(x^*) \leq \tilde{\mathcal{O}}(\frac{\zeta^2}{\mu} + \errk{chain})
\end{align*}
where $\errk{chain}$ was defined in \cref{thm:informal-strong-lsgd-sgd}.  As we shall see, saving the condition number factor on the $\zeta^2$ term in exchange for the $R^{-2}$ factor is tighter for our purposes.

\textbf{2. Choosing between $\hat{x}_0$ and $\hat{x}_{1/2}$:} As discussed in \cref{sec:framework}, it is possible that $F(\hat{x}_{1/2}) > F(\hat{x}_0)$ due to high data heterogeneity between clients.  So we use a stochastic query of $F$ for both $\hat{x}_{1/2}$ and $\hat{x}_0$, and choose the better of the two points based on the query \[\hat{x}_1 \gets \argmin_{x \in \{\hat{x}_{0}, \hat{x}_{1/2}\}} \frac{1}{N \hat{K}} \sum_{i=1}^N \sum_{k=0}^{\hat{K}-1} f(x; \hat{z}_{i,k})\] 

Because we are using a stochastic query of $F$ to determine what to choose for $\hat{x}_1$, we will incur some error.  This error comes from choosing the wrong point based on the stochastic query, i.e. choosing $\hat{x}_0$ when $F(\hat{x}_0) > F(\hat{x}_{1/2})$ or vice versa.  Based on the variance assumption on random queries of $F$, the expected error incurred is $\frac{\sigma}{\sqrt{NK}}$ via an application of Chebyshev's inequality.  Thus, we have that 
\begin{align*}
	\E F(\hat{x}_{1}) - F(x^*) \leq \min \{\frac{\zeta^2}{\mu} + \errk{chain}, \Delta \} + \frac{\sigma}{\sqrt{NK}}
\end{align*}

\textbf{3. Using previous progress for \mbsgd as $\atail$} One could use the convergence rate of \cite{woodworth2020minibatch} which, given $\hat{x}_1$, would have 
\begin{align*}
	&\E F(\hat{x}) - F(x^*) \\
	&\leq \tilde{\mathcal{O}}(\kappa (\E F(\hat{x}_{1}) - F(x^*)) \exp(-\frac{R}{\kappa}) + \frac{\sigma^2}{\mu N K R}) 
\end{align*}
But this loses a condition number factor in the term that only shrinks with $R$, which damages communication round efficiency.  Instead, we follow the analysis of \cite{bottou2018optimization} to obtain
\begin{align*}
	&\E F(\hat{x}) - F(x^*) \\
	&\leq \tilde{\mathcal{O}}((\E F(\hat{x}_{1}) - F(x^*)) \exp(-\frac{R}{\kappa}) + \frac{\kappa \sigma^2}{\mu N K R}) 
\end{align*}
Substituting in the bound for $\E F(\hat{x}_{1}) - F(x^*)$ gives the result from \cref{thm:informal-strong-lsgd-sgd}, and the rate for \chain{\lsgd}{\mbsgd}.  \cref{thm:lsgd-sgd} translates the proof sketch into a formal proof.

Next, we discuss stepsize-decaying (multistage) versions of \chain{\lsgd}{\mbsgd} and \chain{\lsgd}{\asg}.  These algorithms allow one to gradually transition $\ahead$ to $\atail$.  While they do not obtain any convergence rate improvements over their counterparts that do not employ stepsize decay, they can often be performant in practice as observed in our experiments \pcref{sec:experiments} and in the experiments of other works \cite{charles2020outsized} \cite{reddi2020adaptive}.
\begin{theorem}[Informal version of \cref{thm:strong-mlsgd-msgd}]
	\label{thm:informal-strong-mlsgd-msgd}
	Suppose we run \cref{algo:chaining}:
	\begin{enumerate}
		\item Where $\ahead$ is M-\lsgd \pcref{algo:m-lsgd}, a stepsize decaying version of \Lsgd run in stages.  In the first stage $s=1$, choose a stepsize $\eta$, and a number of rounds $R_1$ to run.  Let the stepsize for the $s$-th stage be $\eta_s = \frac{\eta}{2^s}$ and the number of rounds to run for the $s$-th stage be $R_s = \frac{2^s \log(4)}{\mu \eta K}$.
		\item Where $\atail$ is M-\mbsgd \pcref{algo:m-mbsgd}, a stepsize decaying version of \mbsgd run in stages.  In the first stage $s=1$, choose a stepsize $\eta$ (separate from that chosen for $\ahead$), and a number of rounds $R_1$ to run.  Then choose $\eta_s = \frac{\eta}{2^s}$ and $R_s = \frac{2^s \log(4)}{\mu \eta}$.
	\end{enumerate}
	Then this algorithm, if $s$ is constant and $R \geq \kappa$, then this algorithm \chain{M-\lsgd}{M-\mbsgd} has convergence rate 
	\begin{align*}
		&\E F(\hat{x}_2) - F(x^*) \\
		&\leq \tilde{\mathcal{O}}((\min \{\kappa(\kappa (\frac{\zeta^2}{\mu}) + \errk{\lsgd}), \Delta \} + \frac{\sigma}{\sqrt{NK}})\\
		&\times \exp(-\frac{R}{\kappa}) )  + \tilde{\mathcal{O}}(\frac{\kappa \sigma^2}{\mu N K R})
	\end{align*}
\end{theorem}
This is the same rate that is obtained by \chain{\lsgd}{\mbsgd}, except it loses a condition number factor in one of the min terms in the value that's being exponentially decreased.  While the rate is a little bit worse than that of \chain{\lsgd}{\mbsgd}, in practice it can be easier to run, and can be more performant.  We next state the rate for \chain{M-\lsgd}{M-\asg} (the multistage variant of \chain{\lsgd}{\asg}), which has similar relation to the rate of \chain{\lsgd}{\asg}.
\begin{theorem}[Informal version of \cref{thm:m-lsgd-asg}]
	\label{thm:informal-strong-mlsgd-masg}
	Suppose we run \cref{algo:chaining}:
	\begin{enumerate}
		\item Where $\ahead$ is M-\lsgd \pcref{algo:m-lsgd}, a stepsize decaying version of \Lsgd run in stages.  In the first stage $s=1$, choose a stepsize $\eta$, and a number of rounds $R_1$ to run.  Let the stepsize for the $s$-th stage be $\eta_s = \frac{\eta}{2^s}$ and the number of rounds to run for the $s$-th stage be $R_s = \frac{2^s \log(4)}{\mu \eta K}$.
		\item Where $\atail$ is M-\asg \pcref{algo:m-ambsgd}, a stepsize decaying version of \asg run in stages.  In the first stage $s=1$, choose a stepsize $\eta$ (separate from that chosen for $\ahead$), and a number of rounds $R_1$ to run.  Then choose $\eta_s = \frac{\eta}{2^s}$ and $R_s = \frac{2^s \log(4)}{\mu \eta}$.
	\end{enumerate}
	Then this algorithm, if $s$ is constant and $R \geq \sqrt{\kappa}$, then this algorithm \chain{M-\lsgd}{M-\mbsgd} has convergence rate 
	\begin{align*}
		&\E F(\hat{x}_2) - F(x^*) \\
		&\leq \tilde{\mathcal{O}}((\min \{\kappa(\kappa (\frac{\zeta^2}{\mu}) + \errk{\lsgd}), \Delta \} + \frac{\sigma}{\sqrt{NK}})\\
		&\times \exp(-\frac{R}{\sqrt{\kappa}}) ) + \tilde{\mathcal{O}}(\frac{\sigma^2}{\mu N K R})
	\end{align*}
\end{theorem}



==> tables.tex <==
%!TEX root = ./main.tex
\begin{table*}
	\centering
	\renewcommand{\arraystretch}{1.4}
	\caption{ $^\clubsuit$ Algorithm is run after applying gradient minimization technique \cite{nesterov2012make} $^\spadesuit$ for $R \geq \Omega(\kappa)$
	}
	\begin{tabular}{ l l l}
	\hline 
	\textbf{Method/Analysis}  & \textbf{Strongly Convex:}  & \textbf{General Convex:}
	\\ 
	& $\mathbb{E} F(\hat{x}) - F(x^*)  \leq \tilde{\mathcal O}(\cdot)$ &$\mathbb{E} \|\nabla F(\hat{x})\|^2  \leq \tilde{\mathcal O}(\cdot)$ \\
	\hline
	\textit{ Centralized Algorithms} \\
	\hline
	\begin{tabular}{l} 
		\Mbsgd \\
		\asg  \\
	\end{tabular}
	& \begin{tabular}{l}
		$\Delta \exp(-\frac{R}{\kappa})$ { \small\pcref{thm:strongsgd}} 
		\\
		$\Delta \exp(-\frac{R}{\sqrt{\kappa}})$ { \small\pcref{thm:appasg}}
		\\
	\end{tabular}
	& \begin{tabular}{l}
	$\frac{\beta^2 D^2}{R^2}$$^\clubsuit$ 
	\\
	$\frac{\beta^2 D^2}{R^4}$$^\clubsuit$ 
	\end{tabular}
	\\\hline
	\textit{ Federated Algorithms} \\
	\hline
	\begin{tabular}{l}
		SCAFFOLD \\
		\Lsgd \\
		%SCAFFOLD (Theorem \ref{thm:sslsgd}) \\
		\Lsgd $\to$ \Mbsgd \\
		M-\Lsgd $\to$ M-\Mbsgd \\
		\Lsgd $\to$ \asg \\
		M-\Lsgd $\to$ M-ASG  \\
		% Lower bound { \small\citep{woodworth2020minibatch}}
	\end{tabular}
	&
	\begin{tabular}{l}
		$\Delta \exp(- \frac{R}{\kappa})$ { \small \cite{karimireddy2020scaffold}}
		\\
		$ \kappa (\frac{\zeta^2}{\mu})  R^{-2}$ {\small\cite{gorbunov2020local}} \\
		%$\frac{\beta \zeta^2}{\mu^2 R^2}$ \\
		$\min \{\frac{\zeta^2}{\mu} , \Delta \} \exp(-\frac{R}{\kappa})$ { \small \pcref{thm:informal-strong-lsgd-sgd}} \\
		$\min \{\kappa^2(\frac{\zeta^2}{\mu}) , \Delta \}\exp(-\frac{R}{\kappa})$$^\spadesuit$ { \small \pcref{thm:informal-strong-mlsgd-msgd}} \\
		$\min \{\frac{\zeta^2}{\mu} , \Delta \}\exp(-\frac{R}{\sqrt{\kappa}})$ { \small\pcref{thm:informal-strong-lsgd-asg}} \\
		$\min \{\kappa^2(\frac{\zeta^2}{\mu}) , \Delta \}\exp(-\frac{R}{\sqrt{\kappa}})$$^\spadesuit$ { \small\pcref{thm:informal-strong-mlsgd-msgd}} \\
		% $\min\{\frac{\Delta}{\sqrt{\kappa}}, \frac{\mu \zeta^2_*}{\beta^2}\} \exp(-\frac{R}{\sqrt{\kappa}}) + \frac{\sigma^2}{\mu N K R}$ \\
	\end{tabular}
	&
	\begin{tabular}{l}
		$\frac{\beta^2 D^2}{R^2}$$^\clubsuit$  \\
		$\frac{(\beta^{4} \zeta^{5} D^{4})^{2/9}}{R^{10/9}}$$^\clubsuit$  \\
		$\min \{\frac{(\beta^2 \zeta D^{2})^{2/3}}{R^{5/3}}, \frac{\beta^2 D^2}{R^2} \}$  \\
		\\
		$\min \{\frac{(\beta^2 \zeta D^{2})^{2/3}}{R^{8/3}}, \frac{\beta^2 D^2}{R^4} \}$  \\
		\\
	\end{tabular}
	\\\hline 
\end{tabular}
\label{tab:allconvexrates}
\end{table*}
